Product Lines for Service Oriented Applications - PL for SOA

PL for SOA proposes, formally, a software engineering methodology, development techniques and support tools for the provision of service product lines. We propose rigorous modeling techniques for the specification and verification of formal notations and languages for service computing with inclinations of variability. Through these cutting-edge technologies, increased levels of flexibility and adaptivity can be achieved. This will involve developing semantics of variability over behavioural models of services. Such tools will assist organizations to plan, optimize and control the quality of software service provision, both at design and at run time by making it possible to develop flexible and cost-effective software systems that support high levels of reuse. We tackle this challenge from two levels. We use feature modeling from product line engineering and, from a services point of view, the orchestration language Orc. We introduce the Smart Grid as the service product line to apply the techniques to.

==> eptcsdata.tex <==
\providecommand{\firstpage}{34}
\providecommand{\publicationstatus}{L. Kovacs, R.Pugliese, and F. Tiezzi (Eds.): Workshop on\\
Automated Specification and Verification of Web Systems\\
(WWV 2011)\\
EPTCS 61, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.61.3}{10.4204/EPTCS.61.3}}
\pdfoutput=1

